Drone delivery: Reliable Cellular UAV Communication Using Multi-Operator Diversity

The market size of Unmanned Aerial Vehicles (UAVs, a.k.a drones) can reach up to 10% of the global market value. In particular, drone delivery is one of the most attractive applications. The growing number of drones requires appropriate traffic management systems that will rely on cellular networks. However, it has been shown in the literature that these networks cannot provide reliable communication due to low coverage probability and frequent handovers. This article presents a potential solution targeting these problems while requiring no modifications of the existing infrastructure. Namely, equipping the UAV with multiple cellular modems to connect to different providers' networks introduces network diversity resulting in 98% coverage probability at the flight altitude of 100 meters. In contrast, one network ensures only 80% coverage. At the same time, the size of the outage zones becomes up to ten times smaller and the frequency of harmful handovers is reduced to zero. The results are obtained with a physical-layer simulator utilizing a real urban 3D environment, cellular network parameters (e.g., site locations, antenna orientation and gains), and specific aerial channel models.

==> img/boosting/antennas_pcov-tnt.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color2}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
legend pos=south east,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Height [$m$]},
xmin=0, xmax=300,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Coverage Probability, $P_{cov}$},
ymin=0.5, ymax=1,
ytick style={color=black}
]
\addplot [line width=1pt, color0]
table {%
2 0.998066902160645
4 0.99817967414856
6 0.996912479400635
8 0.998326659202576
10 0.999183177947998
12 0.996522545814514
14 0.9952472448349
16 0.993633985519409
18 0.992279529571533
22 0.987971782684326
24 0.986162424087524
28 0.979717016220093
30 0.976979613304138
32 0.973873376846313
34 0.968283772468567
36 0.963197350502014
38 0.95595383644104
40 0.945923328399658
42 0.933133840560913
44 0.927319645881653
46 0.919650673866272
48 0.913374423980713
50 0.905571341514587
52 0.89464259147644
54 0.879684090614319
56 0.870154619216919
58 0.859323263168335
60 0.850031614303589
62 0.83643102645874
64 0.824869275093079
66 0.810786724090576
68 0.790250420570374
70 0.767218112945557
74 0.72751784324646
76 0.708337306976318
78 0.695788860321045
80 0.685919523239136
82 0.674061059951782
84 0.66866660118103
86 0.66872775554657
88 0.667730569839478
90 0.671008348464966
92 0.675866603851318
94 0.685677766799927
96 0.697630643844604
98 0.710294485092163
100 0.715455532073975
102 0.717727780342102
104 0.720188856124878
106 0.721458315849304
108 0.722513914108276
110 0.724699974060059
112 0.726238965988159
114 0.726899981498718
116 0.72468888759613
118 0.72552227973938
120 0.728383302688599
122 0.733322143554688
124 0.738636136054993
126 0.741647243499756
128 0.743933320045471
130 0.744602799415588
132 0.746936082839966
134 0.748333334922791
136 0.749069452285767
138 0.750222206115723
140 0.750783324241638
142 0.752719402313232
144 0.753227710723877
146 0.751608371734619
148 0.747963905334473
150 0.742419481277466
152 0.738224983215332
154 0.736424922943115
156 0.73372220993042
158 0.730613946914673
160 0.727097272872925
162 0.723913908004761
164 0.72124445438385
166 0.718294382095337
168 0.717136144638062
170 0.716519355773926
172 0.715116739273071
174 0.713216662406921
176 0.712191581726074
178 0.7120361328125
180 0.712488889694214
182 0.71387505531311
186 0.715808391571045
190 0.719183325767517
192 0.720597267150879
194 0.721111059188843
196 0.720869421958923
198 0.721475005149841
202 0.726563930511475
204 0.727319478988647
206 0.729094505310059
208 0.730283260345459
212 0.734738826751709
214 0.736552715301514
216 0.737074971199036
218 0.736608266830444
220 0.736344456672668
222 0.735047221183777
224 0.735130548477173
226 0.735655546188354
228 0.735838890075684
230 0.73502779006958
232 0.735116720199585
234 0.734530568122864
236 0.732872247695923
238 0.732088804244995
242 0.733233332633972
244 0.732330560684204
246 0.730402708053589
248 0.729516744613647
250 0.727980613708496
252 0.724211096763611
254 0.72391664981842
256 0.722880601882935
260 0.721252799034119
262 0.719836115837097
264 0.718086123466492
266 0.716716647148132
268 0.716083288192749
270 0.715222239494324
272 0.711897134780884
274 0.71061110496521
276 0.71066951751709
280 0.708444356918335
282 0.708030581474304
284 0.706911087036133
286 0.707052707672119
288 0.706280469894409
290 0.705049991607666
292 0.703333377838135
296 0.696997165679932
298 0.694375038146973
300 0.691933393478394
};
\addlegendentry{Suppressed}
\addplot [line width=1pt, color1]
table {%
2 0.998066902160645
4 0.998192071914673
6 0.996923923492432
8 0.998326659202576
10 0.999189853668213
12 0.996519327163696
14 0.995226144790649
16 0.993622303009033
18 0.992319822311401
22 0.987417101860046
24 0.984716892242432
26 0.979776859283447
28 0.974252700805664
30 0.969120025634766
34 0.960578203201294
36 0.959866285324097
38 0.957806706428528
40 0.955568432807922
42 0.950647830963135
44 0.95033597946167
46 0.951157569885254
48 0.953148245811462
50 0.952253341674805
52 0.955320954322815
54 0.952456712722778
56 0.955282688140869
58 0.961481094360352
60 0.961935639381409
62 0.953181982040405
64 0.952863097190857
66 0.956668972969055
68 0.959557890892029
70 0.957860946655273
72 0.956683158874512
74 0.960016489028931
78 0.959197282791138
80 0.960458278656006
82 0.96251106262207
84 0.962769508361816
86 0.961758375167847
88 0.961005568504333
90 0.958983421325684
92 0.957669496536255
94 0.954633355140686
96 0.950330495834351
98 0.946569442749023
100 0.94308614730835
102 0.940386056900024
104 0.936130523681641
106 0.931530475616455
108 0.927150011062622
110 0.922958374023438
114 0.908766746520996
116 0.900325059890747
118 0.892605543136597
120 0.883066654205322
122 0.873952865600586
124 0.867658376693726
126 0.86169171333313
128 0.856874942779541
130 0.85308051109314
132 0.85004448890686
134 0.847749948501587
136 0.84291672706604
138 0.837863922119141
140 0.833013892173767
142 0.83044445514679
144 0.828747272491455
146 0.828016638755798
148 0.82527494430542
150 0.82033896446228
152 0.81398332118988
154 0.809319496154785
156 0.803933382034302
158 0.799355506896973
160 0.793383359909058
162 0.787152767181396
164 0.780347228050232
166 0.774733304977417
170 0.76538610458374
172 0.761224985122681
176 0.752469420433044
178 0.74970269203186
182 0.747333288192749
184 0.747405529022217
186 0.746688842773438
188 0.746427774429321
190 0.746358394622803
192 0.745727777481079
196 0.742924928665161
198 0.74204158782959
200 0.742444515228271
202 0.743877768516541
204 0.744727849960327
206 0.745869398117065
208 0.746119499206543
210 0.74750828742981
214 0.749308347702026
216 0.749327778816223
220 0.748022198677063
222 0.746799945831299
224 0.74637508392334
226 0.746422290802002
228 0.745816707611084
230 0.744788885116577
232 0.744294404983521
234 0.743611097335815
236 0.741655588150024
238 0.740716695785522
240 0.740619421005249
242 0.740827798843384
244 0.739433288574219
246 0.737458348274231
248 0.736044406890869
250 0.734449982643127
252 0.729949951171875
254 0.729188919067383
256 0.727761030197144
258 0.727088928222656
260 0.726191639900208
262 0.724644422531128
264 0.722533345222473
270 0.719716668128967
272 0.716158390045166
274 0.715283393859863
276 0.714969396591187
278 0.713705539703369
280 0.712611198425293
282 0.712525010108948
284 0.711724996566772
286 0.711669445037842
288 0.710994482040405
290 0.70977783203125
292 0.708088874816895
298 0.698941707611084
300 0.696836113929749
};
\addlegendentry{Normal}
\addplot [line width=1pt, color2]
table {%
2 0.998066902160645
4 0.998192071914673
6 0.996923923492432
8 0.998326659202576
10 0.999186515808105
12 0.996531963348389
14 0.995253324508667
16 0.993628263473511
18 0.992299675941467
22 0.987765073776245
24 0.986201763153076
30 0.975140333175659
32 0.973597526550293
34 0.970098853111267
36 0.970660805702209
38 0.968387007713318
40 0.96716570854187
42 0.962850332260132
44 0.96279239654541
46 0.96725869178772
48 0.972397089004517
50 0.974140644073486
52 0.973591089248657
54 0.972183704376221
56 0.978862524032593
58 0.98145592212677
60 0.978720426559448
62 0.97630763053894
64 0.978805184364319
66 0.980599761009216
68 0.980585813522339
70 0.97991931438446
72 0.979841470718384
74 0.980358242988586
76 0.981924891471863
78 0.982500076293945
80 0.98229444026947
84 0.979305505752563
86 0.976330518722534
88 0.973902702331543
90 0.970755577087402
92 0.96833610534668
94 0.964544415473938
96 0.959952831268311
98 0.956147193908691
102 0.949919462203979
104 0.945524930953979
106 0.941697239875793
110 0.931966662406921
112 0.924375057220459
114 0.917624950408936
116 0.908722162246704
118 0.90108335018158
120 0.891688823699951
122 0.881805539131165
124 0.874000072479248
126 0.867641687393188
128 0.862241744995117
130 0.857822179794312
132 0.854427814483643
134 0.851930618286133
136 0.846697211265564
138 0.841622233390808
140 0.836744427680969
142 0.833630561828613
144 0.83216118812561
146 0.831541657447815
148 0.828861117362976
150 0.824222207069397
152 0.817838907241821
154 0.813263893127441
156 0.807502746582031
158 0.802672147750854
160 0.796447277069092
162 0.790480613708496
164 0.783105611801147
166 0.776927709579468
170 0.76728892326355
172 0.762750029563904
174 0.757952690124512
176 0.753427743911743
178 0.75065553188324
180 0.748797178268433
182 0.747580528259277
184 0.747155547142029
186 0.746569395065308
190 0.746124982833862
192 0.74536669254303
194 0.743955612182617
196 0.742397308349609
198 0.741661071777344
202 0.74334716796875
204 0.743875026702881
206 0.745049953460693
208 0.745155572891235
210 0.746191740036011
212 0.747361183166504
214 0.748119473457336
216 0.748197197914124
218 0.747747182846069
220 0.747002840042114
222 0.745513916015625
224 0.744941711425781
226 0.74483060836792
228 0.744247198104858
230 0.743141651153564
232 0.742827773094177
234 0.741783380508423
236 0.740008354187012
238 0.739119529724121
240 0.739047288894653
242 0.739158391952515
244 0.737955570220947
246 0.735875010490417
248 0.734636068344116
250 0.733105540275574
252 0.728752851486206
256 0.727086067199707
258 0.725927829742432
260 0.725072145462036
262 0.723433256149292
264 0.721391677856445
266 0.720191717147827
268 0.719397306442261
270 0.718444466590881
272 0.715077757835388
274 0.713872194290161
276 0.713750004768372
280 0.711624979972839
282 0.71138334274292
284 0.710147142410278
286 0.710180521011353
288 0.709263801574707
290 0.707963943481445
292 0.706147193908691
296 0.699863910675049
298 0.697091579437256
300 0.694674968719482
};
\addlegendentry{Boosted}
\end{axis}

\end{tikzpicture}


==> img/thresholds/thresholds-org.tex <==
% This file was created with tikzplotlib v0.9.15.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color2}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color3}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Coverage Threshold [dB]},
xmin=-7.675, xmax=7.175,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Coverage Probability, Pcov},
ymin=-0.05, ymax=1.05,
ytick style={color=black}
]
\addplot [line width=0.48pt, color0]
table {%
-7 1
-5 0.999954462051392
-4.5 0.999316692352295
-4 0.994670391082764
-3.5 0.98842978477478
-3 0.978955030441284
-2.5 0.964014053344727
-2 0.943242311477661
-1.5 0.915592432022095
-1 0.876964449882507
-0.5 0.832688093185425
0.5 0.739716649055481
1.5 0.644558906555176
2 0.597503781318665
2.5 0.554138422012329
3 0.511183023452759
3.5 0.469229698181152
4 0.430920600891113
4.5 0.395936727523804
5 0.36491596698761
5.5 0.335124969482422
6 0.307110667228699
6.5 0.282467126846313
};
\addlegendentry{Height: 20 Load: 0.5}
\addplot [line width=0.48pt, color0, dotted]
table {%
-7 0.989204168319702
-6.5 0.979729413986206
-6 0.967749357223511
-5.5 0.948617458343506
-5 0.921331882476807
-4.5 0.887395858764648
-4 0.84412145614624
-3.5 0.799845099449158
-3 0.750102519989014
-2.5 0.699129939079285
-2 0.645105481147766
-1.5 0.595271706581116
-0.5 0.499612808227539
0 0.455290794372559
0.5 0.413702011108398
1 0.377442717552185
1.5 0.345510840415955
2 0.316084384918213
2.5 0.290757536888123
3 0.266478419303894
3.5 0.243793606758118
4 0.223568558692932
4.5 0.204163432121277
5 0.18562388420105
5.5 0.167904138565063
6 0.152234315872192
6.5 0.13934314250946
};
\addlegendentry{Height: 20 Load: 1.0}
\addplot [line width=0.48pt, color1]
table {%
-7 1
-5 0.999644041061401
-4.5 0.994704008102417
-4 0.983889579772949
-3.5 0.967912793159485
-3 0.94726300239563
-2.5 0.921940326690674
-2 0.887405395507812
-1.5 0.84005331993103
-1 0.788562536239624
-0.5 0.735469579696655
0 0.678193092346191
0.5 0.624788522720337
1 0.568891882896423
1.5 0.516466379165649
2 0.467200756072998
2.5 0.41838002204895
3 0.375255823135376
3.5 0.333422303199768
4 0.296840190887451
4.5 0.263106346130371
5 0.233600378036499
5.5 0.211348414421082
6 0.18767249584198
6.5 0.166310667991638
};
\addlegendentry{Height: 40 Load: 0.5}
\addplot [line width=0.48pt, color1, dotted]
table {%
-7 0.981842517852783
-6.5 0.964441537857056
-6 0.939163327217102
-5.5 0.907076120376587
-5 0.862483263015747
-4.5 0.811838030815125
-4 0.760213613510132
-3.5 0.702136158943176
-3 0.638629198074341
-2.5 0.576991558074951
-2 0.51628839969635
-1.5 0.461771249771118
-1 0.415309309959412
-0.5 0.371740102767944
0 0.331864714622498
0.5 0.294080972671509
1 0.260347127914429
1.5 0.230618596076965
2 0.206764578819275
2.5 0.184423685073853
3 0.164218902587891
3.5 0.144993305206299
4.5 0.110057830810547
5 0.0959947109222412
5.5 0.0841121673583984
6 0.0732086896896362
6.5 0.0630173683166504
};
\addlegendentry{Height: 40 Load: 1.0}
\addplot [line width=0.48pt, color2]
table {%
-7 1
-6 0.999911069869995
-5.5 0.997955560684204
-5 0.991555571556091
-4.5 0.969688892364502
-4 0.927111148834229
-3.5 0.864933252334595
-3 0.796800017356873
-2.5 0.718755483627319
-2 0.619422197341919
-1.5 0.526888847351074
-1 0.439066648483276
-0.5 0.365822196006775
0 0.302977800369263
0.5 0.241955518722534
1 0.19213330745697
1.5 0.153333306312561
2 0.123111128807068
2.5 0.0979111194610596
3 0.0772888660430908
3.5 0.0595999956130981
4 0.0444889068603516
4.5 0.0338666439056396
5 0.0264889001846313
5.5 0.020444393157959
6 0.0157778263092041
6.5 0.0119999647140503
};
\addlegendentry{Height: 80 Load: 0.5}
\addplot [line width=0.48pt, color2, dotted]
table {%
-7 0.899111032485962
-6.5 0.830266714096069
-6 0.748533248901367
-5.5 0.649777770042419
-5 0.54746675491333
-4.5 0.45959997177124
-4 0.385955572128296
-3.5 0.324399948120117
-3 0.263466596603394
-2.5 0.2092444896698
-2 0.167066693305969
-1.5 0.133822202682495
-1 0.108711123466492
-0.5 0.0878221988677979
0 0.0701333284378052
0.5 0.0518666505813599
1 0.0404000282287598
1.5 0.0307999849319458
2.5 0.020133376121521
3 0.0152888298034668
3.5 0.011555552482605
4.5 0.00773334503173828
6 0.00337779521942139
6.5 0.00293338298797607
};
\addlegendentry{Height: 80 Load: 1.0}
\addplot [line width=0.48pt, color3]
table {%
-7 1
-6 0.999866724014282
-5.5 0.997022151947021
-5 0.985733270645142
-4.5 0.950977802276611
-4 0.885155558586121
-3.5 0.802888870239258
-3 0.705111026763916
-2.5 0.596266746520996
-2 0.48288893699646
-1.5 0.375555515289307
-1 0.283777713775635
-0.5 0.209111094474792
0 0.155155539512634
0.5 0.115999937057495
1 0.0836888551712036
1.5 0.0625777244567871
2 0.0485333204269409
2.5 0.036622166633606
3 0.0241333246231079
4 0.0108000040054321
4.5 0.00666666030883789
5 0.00311112403869629
5.5 0.00137782096862793
6 0.000311136245727539
6.5 0
};
\addlegendentry{Height: 160 Load: 0.5}
\addplot [line width=0.48pt, color3, dotted]
table {%
-7 0.798222303390503
-6.5 0.695022225379944
-6 0.585022211074829
-5.5 0.472933292388916
-5 0.360222220420837
-4.5 0.267866611480713
-4 0.191333293914795
-3.5 0.137955546379089
-3 0.100488901138306
-2.5 0.0747110843658447
-2 0.0553333759307861
-1.5 0.0412888526916504
-1 0.0300444364547729
-0.5 0.0213778018951416
0 0.0142666101455688
1 0.00435554981231689
1.5 0.0017777681350708
2 0.000755548477172852
3 0
6.5 0
};
\addlegendentry{Height: 160 Load: 1.0}
\end{axis}

\end{tikzpicture}


==> img/thresholds/thresholds-tnt.tex <==
% This file was created with tikzplotlib v0.9.15.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color2}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color3}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Coverage Threshold [dB]},
xmin=-7.675, xmax=7.175,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Coverage Probability, Pcov},
ymin=-0.05, ymax=1.05,
ytick style={color=black}
]
\addplot [line width=0.48pt, color0]
table {%
-7 1
-4.5 0.999817848205566
-4 0.998132348060608
-3.5 0.994715929031372
-3 0.985332250595093
-2.5 0.969525814056396
-2 0.949756383895874
-1.5 0.924474954605103
-1 0.892360925674438
-0.5 0.858834743499756
0 0.823304414749146
0.5 0.787181735038757
1 0.747096061706543
1.5 0.707693696022034
3 0.588165640830994
3.5 0.5513596534729
4.5 0.478795647621155
5 0.444449543952942
6 0.377169370651245
6.5 0.345419764518738
};
\addlegendentry{Height: 20 Load: 0.5}
\addplot [line width=0.48pt, color0, dotted]
table {%
-7 0.997221350669861
-6.5 0.992438316345215
-6 0.980594873428345
-5.5 0.96337628364563
-5 0.936591863632202
-4.5 0.904113292694092
-4 0.868719577789307
-3.5 0.829818248748779
-2.5 0.751469135284424
-2 0.709151387214661
-1.5 0.663235068321228
-1 0.61882209777832
-0.5 0.578235387802124
0.5 0.501571536064148
1 0.465175628662109
1.5 0.430328369140625
2 0.396164536476135
2.5 0.364961504936218
3 0.335535049438477
3.5 0.307930588722229
4 0.279005169868469
4.5 0.251264095306396
5 0.22639274597168
5.5 0.203161239624023
6 0.180795311927795
6.5 0.161845803260803
};
\addlegendentry{Height: 20 Load: 1.0}
\addplot [line width=0.48pt, color1]
table {%
-7 1
-5.5 1
-5 0.999465942382812
-4.5 0.996172666549683
-4 0.986470937728882
-3.5 0.972452163696289
-3 0.948687076568604
-2.5 0.915442824363708
-2 0.87534499168396
-1.5 0.832621335983276
-1 0.788829565048218
-0.5 0.741655588150024
0 0.691499710083008
0.5 0.637249708175659
1 0.583578109741211
1.5 0.528482437133789
2 0.475211381912231
2.5 0.423320055007935
3 0.374543905258179
3.5 0.329684019088745
4 0.286871433258057
4.5 0.248064041137695
5 0.215086817741394
5.5 0.18611478805542
6 0.161281704902649
6.5 0.13920783996582
};
\addlegendentry{Height: 40 Load: 0.5}
\addplot [line width=0.48pt, color1, dotted]
table {%
-7 0.984423637390137
-6.5 0.966800212860107
-6 0.93680465221405
-5.5 0.897730350494385
-5 0.853938579559326
-4.5 0.8084557056427
-4 0.760658740997314
-3.5 0.708722829818726
-3 0.653003931045532
-2.5 0.593369007110596
-2 0.534401416778564
-1.5 0.477347612380981
-1 0.421495318412781
-0.5 0.368446826934814
0 0.321183800697327
0.5 0.280863404273987
1 0.244503736495972
1.5 0.21152651309967
2 0.183088541030884
2.5 0.158923029899597
3 0.138362288475037
3.5 0.120649814605713
4 0.104539394378662
4.5 0.0907431840896606
5.5 0.0659991502761841
6.5 0.0486871004104614
};
\addlegendentry{Height: 40 Load: 1.0}
\addplot [line width=0.48pt, color2]
table {%
-7 0.999555587768555
-6.5 0.996711134910583
-6 0.992222309112549
-5.5 0.981866598129272
-5 0.956755638122559
-4.5 0.911644458770752
-4 0.852222204208374
-3.5 0.784088850021362
-3 0.691377758979797
-2.5 0.583644390106201
-2 0.487733364105225
-1.5 0.411866664886475
-1 0.34755551815033
-0.5 0.292311072349548
0 0.243200063705444
0.5 0.200488924980164
1 0.158400058746338
1.5 0.12755560874939
2 0.103644490242004
2.5 0.0825333595275879
3 0.064977765083313
3.5 0.0493333339691162
4 0.0360444784164429
4.5 0.027377724647522
5 0.019777774810791
5.5 0.0154666900634766
6 0.0116444826126099
6.5 0.00857782363891602
};
\addlegendentry{Height: 80 Load: 0.5}
\addplot [line width=0.48pt, color2, dotted]
table {%
-7 0.833866596221924
-6.5 0.755066633224487
-6 0.643644452095032
-5.5 0.538355588912964
-5 0.452133297920227
-4.5 0.369777798652649
-4 0.307377815246582
-3.5 0.254266738891602
-3 0.210844397544861
-2.5 0.169822216033936
-2 0.135599970817566
-1.5 0.108044385910034
-1 0.0853333473205566
-0.5 0.0669777393341064
0 0.051777720451355
0.5 0.0371555089950562
1 0.0271555185317993
1.5 0.0201777219772339
3 0.00875556468963623
3.5 0.00680005550384521
5 0.00333333015441895
6.5 0.00115561485290527
};
\addlegendentry{Height: 80 Load: 1.0}
\addplot [line width=0.48pt, color3]
table {%
-7 0.999911069869995
-6.5 0.998622179031372
-6 0.996044397354126
-5.5 0.986355543136597
-5 0.954800009727478
-4.5 0.88866662979126
-4 0.81333327293396
-3.5 0.716000080108643
-3 0.60973334312439
-2.5 0.509422302246094
-2 0.403377771377563
-1.5 0.314666628837585
-1 0.242044448852539
-0.5 0.185333371162415
0 0.141377806663513
0.5 0.106977820396423
1 0.0796444416046143
1.5 0.0590221881866455
2 0.0442222356796265
2.5 0.0325777530670166
3 0.02311110496521
3.5 0.0148444175720215
4 0.00951111316680908
4.5 0.00528883934020996
5 0.00284445285797119
6 0.000266671180725098
6.5 0
};
\addlegendentry{Height: 160 Load: 0.5}
\addplot [line width=0.48pt, color3, dotted]
table {%
-7 0.776666641235352
-6.5 0.672533273696899
-6 0.566088914871216
-5.5 0.461111068725586
-5 0.360755562782288
-4.5 0.274488925933838
-4 0.206355571746826
-3.5 0.159199953079224
-3 0.119911074638367
-2.5 0.0892444849014282
-2 0.0682666301727295
-1.5 0.0497332811355591
-1 0.0375111103057861
0 0.0168000459671021
0.5 0.0107555389404297
1 0.00653338432312012
1.5 0.00373327732086182
2 0.00191116333007812
2.5 0.000666618347167969
3 0
6.5 0
};
\addlegendentry{Height: 160 Load: 1.0}
\end{axis}

\end{tikzpicture}

